Bridging Physical Reasoning and Task Generalization via Visual Action Outcome Reasoning Alignment

Vision-language models (VLMs) struggle to generalize in interactive physical reasoning, particularly under unseen tasks and environments. Two key failure modes are prominent: hallucinated chain-of-thought (CoT) reasoning that contradicts physical reality, and misalignment between the model's reasoning and actions. We present VAORA (Visual Action Outcome Reasoning Alignment), a novel reward design that directly addresses both issues. VAORA introduces two complementary rewards: Visual Alignment Reward, which anchors VLM reasoning to the visual context independent of the agent action itself, and Visual-Action Alignment Reward, which grounds reasoning in the visual outcome induced by the model's action. Together, these rewards suppress hallucinated CoT and reduce the gap between reasoning and behavior. To improve training stability, we further employ smooth, dense rewards by estimating success probabilities using a pre-trained in-domain expert agent. Experiments on PHYRE and Virtual Tool support our performances across novel-task and unseen-environment settings, confirming that grounded and generalizable physical intelligence can be induced through VAORA.

==> tables/present.tex <==
\begin{table*}[t]
\small
\centering
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\begin{tabularx}{\textwidth}{LLCCCCCC}
\toprule
\multicolumn{2}{c}{} & \multicolumn{2}{c}{Testing Set 1} & \multicolumn{2}{c}{Testing Set 2} & \multicolumn{2}{c}{Testing Set 3} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
\multicolumn{2}{c}{} & Pass@1 & Pass@5 & Pass@1 & Pass@5 & Pass@1 & Pass@5 \\
\midrule
\multicolumn{8}{l}{\textit{Oracle}} \\
\midrule
\multicolumn{2}{l}{Human} & 0.520 & 0.800 & 0.472 & 0.920 & 0.520 & 0.820 \\
\multicolumn{2}{l}{DQN-expert} & 0.326 & 0.476 & \textbf{0.260} & 0.418 & \textbf{0.338} & 0.466 \\
\midrule
\multicolumn{8}{l}{\textit{Baselines}} \\
\midrule
\multicolumn{2}{l}{Qwen3VL-8B (SFT)} & 0.176 & 0.470 & 0.146 & \underline{0.452} & 0.176 & 0.452 \\
\multicolumn{2}{l}{Gemini-3.1-Pro} & 0.278 & \underline{0.552} & \underline{0.220} & 0.420 & 0.278 & \textbf{0.554} \\
\midrule
\multicolumn{8}{l}{\textit{\textbf{Ours (base model: Qwen3VL-8B-SFT)}}} \\
\midrule
\multicolumn{2}{l}{+EG (Expert-Guided)} & 0.270 & 0.512 & 0.178 & 0.362 & 0.218 & 0.392 \\
\multicolumn{2}{l}{+EG+VAORA} & \textbf{0.382} & \textbf{0.594} & 0.198 & \textbf{0.472} & \underline{0.300} & \underline{0.512} \\
\bottomrule
\end{tabularx}
\caption{\textbf{Results on Phyre test sets.} \ours outperforms all VLM baselines across all three testing sets and surpasses the in-domain DQN expert on the majority of evaluation metrics. \textbf{Bold} and \underline{underline} denote the best and second-best results (excluding human), respectively.}
\label{tab:phyre_main}
\vspace{-6mm}
\end{table*}

\begin{table*}[t]
\small
\centering
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\begin{tabularx}{\textwidth}{LLCCC}
\toprule
\multicolumn{2}{c}{} & Pass@1 & Pass@3 & Pass@5 \\
\midrule
\multicolumn{2}{l}{Human} & 0.333 & 0.661 & 0.778 \\
\midrule
\multicolumn{2}{l}{DQN-expert (phyre)} & 0.000 & 0.056 & 0.056 \\
\midrule
\multicolumn{2}{l}{Qwen3VL-8B (SFT)} & 0.0 & 0.167 & 0.222 \\
\multicolumn{2}{l}{Gemini-3.1-Pro} & \underline{0.111} & \textbf{0.278} & \textbf{0.389} \\
\midrule
\multicolumn{5}{l}{\textit{\textbf{Ours (base model: Qwen3VL-8B-SFT)}}} \\
\midrule
\multicolumn{2}{l}{+EG+VAORA} & \textbf{0.167} & \underline{0.222} & \underline{0.333} \\
\bottomrule
\end{tabularx}
\caption{\textbf{Results on Virtual-Tool.} \ours achieves the best Pass@1 and remains competitive with frontier closed-source VLMs on Pass@3 and Pass@5, despite never being exposed to Virtual-Tool during training.}
\label{tab:virtual_tool}
\vspace{-3mm}
\end{table*}

\begin{table*}[t]
\footnotesize
\centering
\setlength{\tabcolsep}{4pt}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{tabularx}{\textwidth}{lCCCCCC}
\toprule
Method & Descriptive & Counterfactual & Enable & Causal & Prevent & \textbf{Overall} \\
\midrule
Qwen3-VL-8B-Instruct & 26.60 & 41.70 & 40.70 & 42.00 & 40.70 & 38.34 \\
SFT & 37.70 & 46.90 & 43.90 & 44.70 & 47.50 & 44.14 \\
+EG+VAORA & \textbf{39.40} & \textbf{48.20} & \textbf{46.30} & \textbf{45.90} & \textbf{50.50} & \textbf{46.06} \\
\bottomrule
\end{tabularx}
\caption{\textbf{CRAFT VQA Benchmark Performance.} Training exclusively on PHYRE, \ours achieves consistent improvement across all CRAFT VQA question types, validating that the learned physical reasoning transfers beyond the interactive training environment.}
\label{tab:CRAFT_VQA}
\vspace{-6mm}
\end{table*}
